State Constrained Stochastic Optimal Control Using LSTMs

In this paper, we propose a new methodology for state constrained stochastic optimal control (SOC) problems. The solution is based on past work in solving SOC problems using forward-backward stochastic differential equations (FBSDE). Our approach in solving the FBSDE utilizes a deep neural network (DNN), specifically Long Short-Term Memory (LSTM) networks. LSTMs are chosen to solve the FBSDE to address the curse of dimensionality, non-linearities, and long time horizons. In addition, the state constraints are incorporated using a hard penalty function, resulting in a controller that respects the constraint boundaries. Numerical instability that would be introduced by the penalty function is dealt with through an adaptive update scheme. The control design methodology is applicable to a large class of control problems. The performance and scalability of our proposed algorithm are demonstrated by numerical simulations.

==> derivation.tex <==
\section{Problem Formulation}
A system with dynamics that involves stochastic processes can be described using a stochastic differential equation (SDE), which has the form of,
 \begin{equation}
    \label{eq:SDE1}
    dx(t) = f(x(t),t)dt +\sigma(x(t),t)dw(t),
\end{equation}
with initial condition $x(0) = x_0$ and $w(t)$ being a standard Brownian motion. Here we have the state $x\in\mathbb{R}^n$, time $0<t<T<\infty$, $f: \mathbb{R}^n\times[0, T]\rightarrow\mathbb{R}^n$ represents the drift,  $\sigma: \mathbb{R}^n\times[0, T]\rightarrow\mathbb{R}^n$ represents the diffusion. The solution to~\eqref{eq:SDE1} is a stochastic process $(x(t))_{t\geq 0}$ that satisfies this system. In many cases we are more interested in $dg(x(t), t)$, where $g(\cdot)$ is a function of $x(t)$ and $t$. By defining the \textit{generator} of $x(t)$ with $\mathcal L(\cdot)$, where $dx(t)$ is defined in \eqref{eq:SDE1}, as 
\begin{equation}
    \mathcal{L}(\cdot) = f(x,t) \frac{\partial(\cdot)}{\partial x} + \frac{1}{2}\sigma^2(x,t)\frac{\partial^2(\cdot)}{\partial x^2},
\end{equation}
we can obtain the derivative of $g(x(t), t)$  using It\={o}'s Lemma which states,
\begin{equation}
\begin{aligned}
\label{eq:ito}
    dg(x(t),t) =& \left(g_t(x(t),t) + \mathcal{L}g(x)\right)dt +\\
                &\ \sigma(x(t),t)g_x(x(t),t)dw(t).
\end{aligned}
\end{equation}
In a multivariate setting, the generator is defined as,
\begin{equation}
    \mathcal{L}g = \frac{1}{2}\hbox{trace}(\Sigma\Sigma^T g_{xx}) + f^Tg_x,
\end{equation}
and It\=o's lemma becomes,
\begin{equation}
\begin{aligned}
dg(x(t), t) =& g_t(x(t), t)dt + \mathcal{L}g(x(t), t)dt +\\
             &\ (\sigma(x(t),t)g_x(x(t), t))^Tdw(t).
\end{aligned}
\end{equation}
This gives us the result known as Dynkin's formula,
\begin{equation}
\begin{aligned}
&\lim_{\Delta t\searrow 0}\mathbb E\left[\frac{g(x(t+\Delta t),t+\Delta t) -g(x,t)}{\Delta t}\Big|x(t)= x\right]\\
=& g_t(x,t)+ \mathcal L g(x,t).
\end{aligned}
\label{eq:dynkins}
\end{equation}
If we have the value function for \eqref{eq:SDE1} as,
\begin{equation}
    v(x,t) = \mathbb E\left[g(x(T))+\int_t^Tq(x(s))ds\Big|x(t) = x\right],
\end{equation}
where we take $g$ and $q$ to be a function only of $x$ and not $t$.
Then, using Bellman's principle along with Dynkin's formula from \eqref{eq:dynkins}, we can have,
\begin{subequations}
\begin{align}
    -q(x) &=\lim_{\Delta t\searrow 0}\mathbb E\left[\frac{v(x(t+\Delta t),t+\Delta t) -v(x,t)}{\Delta t}\Big|x(t)= x\right]\\
                           &= v_t(x,t)+ \mathcal L v(x,t),
\end{align}
\end{subequations}
which means $v(x,t)$ is the solution of a partial differential equation (PDE) given the boundary condition,
\begin{align}
	\label{eq:PDE1}
	v_t(x(t), t) + \mathcal{L}v(x(t), t) + q(x(t))&= 0\\
	\nonumber
	v(x(T),T) &= g(x(T)),
\end{align}
this is called the Feynman-Kac formula. For a controlled SDE,
\begin{equation}
	\label{eq:SDE2}
	dx(t) = f(x(t),t)dt +G(x(t),t)u(t)dt+\Sigma(x(t),t)dw(t),
\end{equation}
where $u(\cdot)$ is the control input. A stochastic control problem may have the following minimization objective $J^u(x,t)$ equal to,
\begin{equation}
    \mathbb E\left[g(x(T)) + \int_t^T\left(q(x(s))+\frac{1}{2}u(s)^TRu(s)\right)ds\Big|x(t) = x\right],
\end{equation}
and the value function for the optimal control is defined as, 
\begin{equation}
    V(x,t) := \inf_{u\in\mathcal U} J^u(x,t).
\end{equation}
Using Dynkin's formula along with Bellman's principle we can have,
\begin{equation}
    q(x)-\frac{1}{2}u^TRu \leq V_t(x,t) + \mathcal L V(x,t)+(Gu^*)^TV_x,
\end{equation}
with equality only for the optimal control $u^*$, which yields the Hamilton-Jacobi-Bellman (HJB) equation,
\begin{subequations}
\begin{align}
&\begin{aligned}
    &V_t(x,t) +\mathcal{L}V(x,t)+\\ &\min_u\Big(q(x)+(G(x,t)u)^TV_x(x,t)+\frac{1}{2}u^{T}Ru\Big) = 0
\end{aligned}\\
	&V(x,T) = g(x).
\end{align}
\label{eq:HJB}
\end{subequations}
Denote the Hamiltonian as
\begin{equation}
    h(x,V_x,t) = \min_u\left(q(x)+(G(x,t)u)^TV_x(x,t)+\frac{1}{2}u^TRu\right).
\end{equation}
Using first-order conditions to solve for the optimal control in the Hamiltonian gives us,
\begin{equation}
	\label{eq:feedbackForm}
	\mathbf{u}(x,t) = R^{-1}G^T(x,t)V_x(x,t)\ ,
\end{equation}
and the Hamiltonian can be expressed as
\begin{equation}
    h(x, V_x, t) = q(x)-\frac{1}{2}\left\|R^{-1/2}G^T(x,t)V_x(x, t)\right\|^2.
\end{equation}
We define $G(x(t), t) = \Sigma(x(t), t)\Gamma(x(t), t)$, we can write~\eqref{eq:SDE2} as,
\begin{equation}
    dx(t) = f(x(t),t)dt + \Sigma(x(t), t)\bigg(\Gamma(x(t), t)u(t)dt + dw(t)\bigg).
\end{equation}
Then we can define a change of measure as,
\begin{equation}
    d\tilde w(t) = \Gamma(x(t),t)u(x(t),t)dt + dw(t).
\end{equation}
By satisfying the Novikov condition,
\begin{equation}
    \mathbb{E}\Bigg[\exp\left( \frac{1}{2}\int_0^T\left\|\Gamma(x(t),t)u(t)\right\|^2dt\right)\Bigg]<\infty
\end{equation}
we can say that the Radon-Nikodym derivative is a martingale which confirms there exists a change of measure and $\tilde w(t)$ is a standard Brownian motion under this new measure. We can define,
\begin{subequations}
\label{eq:BSDErepresentation}
\begin{align}
	y(t) &:= V(x(t),t)\\
	z(t) &:= \Sigma^T(x(t),t)V_x(x(t),t).
\end{align}
\end{subequations}
In the spirit of Feynman-Kac lemma we write the implicit solution to~\eqref{eq:HJB} under the optimal control as
\begin{equation}
\begin{aligned}
    \label{eq:implicitFeynmanKac}
	y(x,t) &= \widetilde{\mathbb E}\left[g( x(T))+\int_t^Th(x(s), z(s), s)ds \Big| x(t) =x\right]\\
	s.t.\ dx & = f(x(t),t)dt + \Sigma(x(t),t)d\tilde w(t).
\end{aligned}
\end{equation}
Then by applying It\=o's lemma to $y(t)$ we have,
\begin{equation}
    dy(t) = \left(V_t( x(t),t) +\mathcal LV( x(t),t) \right)dt + z^T(t)d\tilde w(t)
\end{equation}
but using the HJB equation of \eqref{eq:HJB}, we see that $V_t +\mathcal LV = -h$, which we use to obtain the backward stochastic differential equation (BSDE) for the optimal value function,
\begin{subequations}
\label{eq:BSDE}
\begin{align}
	-dy(t) &= h(x(t),z(t),t)dt - z^T(t)d\tilde w(t)\\
	y(T) &=g(x(T)),
\end{align}
\end{subequations}
the corresponding forward stochastic differential equation (FSDE) is,
\begin{subequations}
\label{eq:FSDE}
\begin{align}
    dx(t) & = f(x(t),t)dt + \Sigma(x(t),t)d\tilde w(t)\\
	x(0) &= x_0,
\end{align}
\end{subequations}
By undoing the change of measure in~\eqref{eq:BSDE} and~\eqref{eq:FSDE} we can have,
\begin{subequations}
\label{eq:FBSDE_undo}
\begin{align}
-dy(t) &= \begin{aligned}
&\left(h(x(t),z(t),t) -z^T(t)\Gamma(x(t),t)u(x(t),t)\right)dt\\
&- z^T(t)dw(t)
\end{aligned}\\
dx(t) &= \begin{aligned}
&\left(f(x(t),t) +\Sigma(x(t),t)\Gamma(x(t),t)u(x(t),t)\right)dt\\
&+ \Sigma(x(t),t)dw(t)
\end{aligned}\\
y(T) &= g(x(T))\\
x(0) &= x_0,
\end{align}
\end{subequations}
which is in the form of a forward-backward stochastic differential equation (FBSDE).
